The Effectiveness of Haptic Properties Under Cognitive Load: An Exploratory Study

With the rise of wearables, haptic interfaces are increasingly favored to communicate information in an ambient manner. Despite this expectation, existing guidelines are developed in studies where the participant's focus is entirely on the haptic task. In this work, we systematically study the cognitive load imposed by properties of a haptic signal. Participants wear a haptic device on their forearm, and are asked to perform a 1-back task. Each experimental condition isolates an individual property of the haptic signal (e.g., amplitude, waveform, rhythm) and participants are asked to identify the gradient of the data. We evaluate each condition across 16 participants, measuring participants' response times, error rates, and qualitative and quantitative surveys (e.g., NASA TLX). Our results indicate that gender and language differences may impact preference for some properties, that participants prefer properties that can be rapidly identified, and that amplitude imposes the lowest cognitive load.

==> sections/figures.tex <==
\section{Figures}


% \begin{table}[t]
%     \small
%     \centering
%     \csvautobooktabular{figures/Kruskal_Time_Table.csv}
%     \caption{P-value Summary from Post hoc Pairwise Comparisons Using Wilcoxon Signed Rank Test with Holm Adjustment}
%     \label{table:Kruskal_Time_Table}
% \end{table}

% \begin{figure*}
% \begin{center}
% \begin{floatrow}
% \ffigbox{%
%   \includegraphics[width=\columnwidth]{figures/1_Diff_in_Time_by_Condition.pdf}
% }{%
%   \caption{Response Time Differences by Gender across Conditions}%
%   \label{fig:Time_Differences}
% }
% \capbtabbox{%
%   \small
%   \csvautobooktabular{figures/Time_Table.csv}
% }{%
%   \caption{Response Time Differences by Gender across Conditions}%
%   \label{table:Time_Table}
% }
% \end{floatrow}
% \end{center}
% \end{figure*}

% \begin{figure}[t]
%     \includegraphics[width=\columnwidth]{figures/1_Diff_in_Time_by_Condition.pdf}
%     \caption{Response Time Differences by Gender across Conditions}
%     \label{fig:Time_Differences}
% \end{figure}

% \begin{table}[t]
%     \small
%     \centering
%     \csvautobooktabular{figures/Time_Table.csv}
%     \caption{Response Time Differences by Gender across Conditions}
%     \label{table:Time_Table}
% \end{table}

% \begin{figure}[b]
%     \centering
%     \includegraphics[width=7cm]{figures/2_Diff_in_1back_by_Condition.pdf}
%     \caption{1-back Task Scores}
%     \label{fig:1_back_Scores}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=7 cm]{figures/3_Diff_in_haptic_by_Condition.pdf}
%     \caption{Haptic Gradient Detection Scores}
%     \label{fig:Haptic_Scores}
% \end{figure}

% \begin{table*}[h]
%     \small
%     \centering
%     \csvautobooktabular{figures/Haptic_Table.csv}
%     \caption{Scores across Conditions by Gender in the Haptic Gradient Detection Task}
%     \label{table:Haptic_Table}
% \end{table*}


% \begin{figure*}[h]
%     \centering
    
%     \begin{subfigure}
%         \centering
%         \includegraphics[width=2.2in]{figures/4_Likert_Q1_Mental.pdf}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}
%         \centering
%         \includegraphics[width=2.2in]{figures/5_Likert_Q2_Rushed.pdf}
%     \end{subfigure}
    
%     \begin{subfigure}
%         \centering
%         \includegraphics[width=2.2in]{figures/6_Likert_Q3_Success.pdf}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}
%         \centering
%         \includegraphics[width=2.2in]{figures/7_Likert_Q4_Difficulty.pdf}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}
%         \centering
%         \includegraphics[width=2.2in]{figures/8_Likert_Q5_Stress.pdf}
%     \end{subfigure}
    
%     \label{fig:NASA-TLX Results} 
%     \caption{NASA-TLX Responses by Gender across Conditions}
% \end{figure*}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=8.5cm]{figures/9_Pre_Post_Difficulty.pdf}
%     \caption{Difficulty Perception Before and After Combining the Haptic Gradient Detection Task}
%     \label{fig:before_after_difficulty}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=8.5cm]{figures/10_RolledTime_per_Trial.pdf}
%     \caption{Response Times across Trials}
%     \label{fig:rolling_time}
% \end{figure}







==> sections/summary_of_results.tex <==
\subsection{Summary}
The three measures collected from the experiment were the response time data from the n-back task, the performance score on the n-back task, and the performance score on the up/down haptic task. We consider the response time in the n-back task to be a good indicator of cognitive load imposed on the participant by the haptic condition. 

The analysis of the results for all participants showed that the response time for amplitude was significantly shorter than rhythm and waveform. Amplitude was followed by duration which was significantly shorter than rhythm as well. Although we did not find any statistically significant results on the performance score on the n-back task and on the haptic task, we observed a visual trend showing that participants performed best on both tasks with the amplitude and duration condition. Interestingly, the participant preference on the NASA-TLX survey validated this finding. Participants found amplitude to be the condition ranked as least demanding and most successful, and one where the participant had to work the least hard and was the least insecure. 

On the other hand, for all participants, while not statistically significant, our results revealed that waveform followed by rhythm were the two conditions the participants took the longest to complete. We also found rhythm and spatio-temporal pattern to be the lowest score on the n-back task, and rhythm, waveform, and spatio-temporal pattern (in that order) to be the fairly close lowest scores on the haptic task. This finding also aligned with the NASA-TLX results where waveform and spatio-temporal pattern ranked as the highest mental demand, and waveform was ranked as the least successful and most difficult. 


